Electric conductivity in non-Hermitian holography

We study the phase structure and charge transport at finite temperature and chemical potential in the non-Hermitian PT-symmetric holographic model of arXiv:1912.06647. The non-Hermitian PT-symmetric deformation is realized by promoting the parameter of a global U(1) symmetry to a complex number. Depending on the strength of the deformation, we find three phases: stable PT-symmetric phase, unstable PT-symmetric phase, and an unstable PT-symmetry broken phase. In the three phases, the square of the condensate and also the spectral weight of the AC conductivity at zero frequency are, respectively, positive, negative, and complex. We check that the Ferrell-Glover-Tinkham sum rule for the AC conductivity holds in all the three phases. We also investigate a complexified U(1) rotor model with PT-symmetric deformation, derive its phase structure and condensation pattern, and find a zero frequency spectral weight analogous to the holographic model.

==> backup/analytical_part.tex <==
\subsubsection{Small $N/T$}

In this subsection, we derive analytically the electrical conductivity when $N\ll T$. Although any of the results derived here can be generalized to any $\Delta<d$ and $v$, the resulting expressions become cumbersome. Hence, and also in the aim to compare these results with the numeric approach, we keep the same values for these parameters as in previous sections. 
\DRF{Zhuo-yu: can you explain this issue about neglecting $\phi^2$ corrections to the background fields, but not in this equation?. I remember that the responsible was the $G_N$ constant.}


After inspecting \ref{ODEax}, we notice that via the field redefinition
\begin{equation}
    a(z) = \frac{\alpha(z)}{\sqrt{z_h^3 - z^3}}\,,
\end{equation}
the equation \ref{ODEax} is recast into a Schrödinger equation of the form
\begin{equation}
    \alpha'' + \mathcal{V} \alpha = 0 \,,\quad \mathcal{V} = \frac{-3 z^4+12 z z_h^3+4 \omega ^2 z_h^6}{4 \left(z^3-z_h^3\right)^2}-\frac{2 q^2 s z_h^3 \phi^2}{z^5-z^2 z_h^3} \,.
\end{equation}

This enables us to identify the ''probability current'', $\mathcal{J}$
\begin{equation} 
    \mathcal{J}(z) = \alpha'(z)\overline{\alpha}(z) - \overline{\alpha'(z)}\alpha(z)\,,
\end{equation}
which is conserved on-shell, i.e. $ \frac{d}{dz} \mathcal{J} = 0$, leading to the condition 
\begin{equation} \label{eq:jcons}
    \mathcal{J}_B = \mathcal{J}\vert_{z\to 0} = \mathcal{J}\vert_{z\to z_h} = \mathcal{J}_H\,.
\end{equation}
The ''current'' $\mathcal{J}$ is likely related to the membrane-paradigm, as it allows to connect boundary coefficients to horizon quantities. It is also closely related to Ward identities in holography and a procedure to retrieve it in general gravity duals with parity symmetry has been derived in \cite{Hoyos_2016}. At this point, we examine the two asymptotic regimes separately. Firstly, near the boundary, we find that 
\begin{equation} \label{eq:axprobenb}
   \alpha\vert_{z\to 0}  \sim \alpha_{(0)} + \alpha_{(1)}z\,.
\end{equation}
Note that the normalizable coefficient $\alpha_{(1)}$ is not independent from the $\alpha_{(0)}$ coefficient. Indeed, ingoing boundary conditions at the horizon of the form \ref{Regax} impose a relation between the boundary normalizable and non-normalizable modes,
\begin{equation}
\alpha_{(1)} = g(\omega) \alpha_{(0)}\,.
\end{equation}
Moreover, at $z\sim z_h$, a solution which satisfies the ingoing boundary condition \ref{Regax} is given by
\begin{equation} \label{eq:axprobenh}
    \alpha\vert_{z\to z_h} \sim \alpha_H = A_H \sqrt{z_h -z}  \Gamma
   \left(1-\frac{2 i z_h\omega }{3}\right) \sqrt{9 N^2 q^2 s z_h^2 \Gamma\left(\frac{2}{3}\right)^6+\pi ^2 \left(4 \omega ^2 z_h^2+9\right)} \, \mathcal{I}\left(\omega\right)
\end{equation}
where $\mathcal{I}(\omega)$ is the modified Bessel function $I_n(x)$ of the first kind, whose arguments are given by
\begin{equation}
   \mathcal{I}(\omega) =  I_{-\frac{2}{3} i z_h \omega }\left(i\frac{\sqrt{z-z_h} \sqrt{8 \pi ^2 \omega ^2
   z_h^2+18 N^2 q^2 s \Gamma \left(\frac{2}{3}\right)^6 z_h^2+18 \pi ^2}}{3 \pi }\right)\,.
\end{equation}

In some limits, we can consider $\alpha_H(z)$ as the full expression holding in the whole domain, so the Green function is 
\begin{align}
&G_R(\omega)=i\left[\frac{3i+2z_h\omega}{6z_h}-\right. \nonumber\\
&\left.\frac{I_{1-\frac23 i z_h\omega}\left(\frac{i\sqrt{z_h}\sqrt{2\pi^2(9+4z_h^2\omega^2)+18N^2q^2s z_h^2\Gamma(\frac23)^6}}{3\pi}\right)}{I_{-\frac23 i z_h\omega}\left(\frac{i\sqrt{z_h}\sqrt{2\pi^2(9+4z_h^2\omega^2)+18N^2q^2s z_h^2\Gamma(\frac23)^6}}{3\pi}\right)}\cdot\frac{\sqrt{2\pi^2(9+4z_h^2\omega^2)+18N^2q^2s z_h^2\Gamma(\frac23)^6}}{6\pi z_h^{1/2}}\right]
\end{align}
For pure AdS case, we have the solution 
\begin{align}
a(z)=A\,e^{i\frac{\sqrt{3}}{3}z_h\omega\arctan(\frac{2z+z_h}{\sqrt{3}z_h})}(z^2+z_hz+z_h^2)^{\frac{i}{6}z_h\omega}(z_h-z)^{-\frac{i z_h\omega}{3}}
\end{align}

Expnding \ref{eq:axprobenh} near the horizon, we find 
\begin{equation} \label{eq:alphanh}
\alpha_H \sim A_H \left(12 \pi^2\right)^{\frac{i \omega z_h}{3}} \Bigg\lbrace\left(z_h -z\right) \left[9 N^2 q^2 s z_h^2 \Gamma
   \left(\frac{2}{3}\right)^6+\pi ^2 \left(4 \omega^2 z_h^2+9\right)\right]\Bigg\rbrace^{1/2 -i \omega z_h/3}
\end{equation} 
where $A_H$ is some normalization constant. Combining \ref{eq:axprobenb} and \ref{eq:axprobenh} with \ref{eq:jcons}, we find
\begin{equation}\label{eq:g}
    g -\overline{g} \equiv 2i \, {\rm Im}[g] = \frac{2}{3} i \vert A_H\vert^2 w \left(\frac{9 N^2 q^2 s z_h^2 \Gamma\left(\frac{2}{3}\right)^6}{\pi^2 \left(4 \omega^2 z_h^2 +9\right)}+1\right)\,.
\end{equation}

In principle, there is freedom to choose the normalization constant $A_H$. We opted fix it by matching the $N\to 0$ limit of \ref{eq:g} with the pure AdS solution for $a_1$, which can be derived analytically throughout the whole radial coordinate 
\begin{equation}\label{eq:a1ads}
   a_{\rm AdS} \sim  3^{\frac{i \omega z_h}{6}} e^{\frac{1}{18} i \left(3+2\sqrt{3} \pi \right) \omega z_h} (z_h-z)^{-\frac{i \omega z_h}{3}}\,,
\end{equation}
in such a way that \ref{eq:alphanh} smoothly connects to \ref{eq:a1ads} in absence of a scalar field. After this, we find
\begin{equation}\label{eq:a1ads}
{\rm Im}[g] =  w \left[1+\frac{9 N^2 q^2 s z_h^2 \Gamma\left(\frac{2}{3}\right)^6}{\pi^2 \left(4 \omega^2 z_h^2 +9\right)}\right]\,.
\end{equation}

The full retarded Green function $G_R$ can be obtained by following \ref{eq:Gr}, which reads
\begin{equation} \label{eq:GRprobe}
    G_R(\omega) = i \omega + \frac{9 N^2 q^2 s \Gamma \left(\frac{2}{3}\right)^6}{4 \pi ^2 (2 \pi  T- i \omega )}\,.
\end{equation}

To compute the conductivity, we need to evaluate the formula \ref{eq:sigma}. This can be done by applying the Sokhotski–Plemelj theorem, 
\begin{equation} 
\lim_{\delta\to 0} \frac{1}{x+\delta i} = \mathcal{P}\left[\frac{1}{x}\right] -i \pi \delta(x)\,,
\end{equation} 
where $\mathcal{P}$ stands for the principal value. After this, we find
\begin{equation}\label{eq:sigmaprobe}
\sigma = \left[1 +\frac{9 N^2 q^2 s \Gamma
   \left(\frac{2}{3}\right)^6}{4 \pi^2 \left(4 \pi ^2 T^2+\omega
   ^2\right)} - \frac{9 N^2 q^2 s \Gamma
   \left(\frac{2}{3}\right)^6}{8 \pi^2 T}\delta\left(\omega\right) \right] - i  \frac{9 N^2 q^2 s T \Gamma\left(\frac{2}{3}\right)^6}{2\pi\omega\left(4\pi^2 T^2+\omega^2\right)}  \,.
\end{equation} 
From \ref{eq:sigmaprobe}, it is straightforward to compute the weight spectral distribution, which reads
\begin{equation} 
W(\omega) = \frac{9 N^2 q^2 s \Gamma \left(\frac{2}{3}\right)^6}{8 \pi ^2 T} F(\omega) \,, \quad F(\omega) = 1+ \frac{1}{\pi}\cot ^{-1}\left(\frac{2 \pi  T}{\omega }\right) -2\theta(\omega)
\end{equation} 
where $\theta(\omega)$ stands for the Heavyside function. In particular, $F<0 \,\forall \,\omega>0$, so the overall sign of $W$ is determined by $s$ alone. In particular, when $x>1$, $W<0$ and $>0$ if otherwise. Furthermore, the sum rule, 
\begin{equation} \label{eq:intresigma}
    \int^\infty_{-\infty} \big\lbrace {\rm Re}[\sigma] - 1 \big\rbrace \, d\omega = 0\,,
\end{equation}
is always satisfied. Moreover, notice that it requires a finite coupling strength between the gauge field and the scalar field, i.e. $q\neq 0$ in order to see any scalar field contribution to the longitudinal conductivity \ref{eq:sigmaprobe}, as expected. 














This fact alone suggests that more general mechanisms are behind it. In \cite{Coleman:manybody}, it was suggested that this law arises as a natural consequence of Newton's law, i.e. 
 \begin{align}
        \frac{J(t=0^+)}{E}
        =\sigma(t=0^+)
        =\int_{-\infty}^{\infty} \frac{d\omega}{2\pi} \sigma(\omega+i0^+) e^{-i\omega 0^+}
        =\int_{-\infty}^{\infty} \frac{d\omega}{\pi} \Re\sigma(\omega)
\end{align}
For such a short time evolution, the non-unitary  is not important. Even for an open system, such as the Fermi liquid or superfluid coupled to the environment, the sum rule should not been violated. \DRF{I think we need to explain it in other way though, any suggestions?...}

\section{Small $N/T$}

\zycom{In this appendix, we explore to derive the electrical conductivity in the probe limit and $N\ll T$ limit analytically. The probe limit is realized by recovering the Newton's constant $G_N$ in the action \eqref{action}, namely, $R+d(d-1)/L^2\to \frac1{G_N}(R+d(d-1)/L^2)$, and then require $G_N\to0$.} Although any of the results derived here can be generalized to the cases for any $\Delta<d$ and $v$, the resulting expressions will manifest cumbersome. Hence, we maintain the same values for these parameters as in previous sections for simplicity of expressions as well as to compare these results with the numerical ones, 
\DRF{Zhuo-yu: can you explain this issue about neglecting $\phi^2$ corrections to the background fields, but not in this equation?. I remember that the responsible was the $G_N$ constant.} After inspecting \ref{ODEax}, we notice that via the field redefinition
\begin{equation}
a(z) = \frac{\alpha(z)}{\sqrt{z_h^3 - z^3}}\,,
\end{equation}
the equation \ref{ODEax} can thus be recast into a Schrödinger equation of the form
\begin{equation}
\alpha''(z) + \mathcal{V}(z) \alpha(z) = 0 \,,\quad \mathcal{V}(z) = \frac{-3 z^4+12 z z_h^3+4 \omega ^2 z_h^6}{4 \left(z^3-z_h^3\right)^2}-\frac{2 q^2 s z_h^3 \phi(z)^2}{z^5-z^2 z_h^3} \,.
\end{equation}
This enables us to construct the conservative ``probability current'' $\mathcal{J}(z)$
\begin{equation} 
\mathcal{J}(z) = \alpha'(z)\overline{\alpha(z)} - \overline{\alpha'(z)}\alpha(z)\,,
\end{equation}
satisfying $ \frac{d}{dz} \mathcal{J} = 0$, which leads to the following relation
\begin{equation} \label{eq:jcons}
    \mathcal{J}_B = \mathcal{J}\vert_{z\to 0} = \mathcal{J}\vert_{z\to z_h} = \mathcal{J}_H\,.
\end{equation}
The ``current'' $\mathcal{J}$ is likely related to the membrane-paradigm, as it allows to connect boundary coefficients to horizon quantities. It is also closely related to Ward identities in holography and a procedure to retrieve it in general gravity duals with parity symmetry has been derived in \cite{Hoyos_2016}. At this point, we examine the two asymptotic regimes separately. Firstly, near the boundary, we find that 
\begin{equation} \label{eq:axprobenb}
   \alpha\vert_{z\to 0}  \sim \alpha_{0} + \alpha_{1}z\,.
\end{equation}
Note that the normalizable coefficient $\alpha_{1}$ is dependent on the coefficient $\alpha_{0}$. Indeed, ingoing boundary conditions at the horizon of the form \ref{Regax} impose a relation between the boundary normalizable and non-normalizable modes,
\begin{equation}
\alpha_{1} = G_R(\omega)\alpha_{0}\,.
\end{equation}
Moreover, near the horizon, a solution which satisfies the ingoing boundary condition \ref{Regax} is given by
\begin{equation} \label{eq:axprobenh}
\alpha_h(z)=A_h \sqrt{z_h -z}  \Gamma
   \left(1-\frac{2 i z_h\omega }{3}\right) \sqrt{9 N^2 q^2 s z_h^2 \Gamma\left(\frac{2}{3}\right)^6+\pi ^2 \left(4 \omega ^2 z_h^2+9\right)} \, \mathcal{I}\left(\omega\right)
\end{equation}
where $\mathcal{I}(\omega)$ is the modified Bessel function $I_n(x)$ of the first kind, whose arguments are given by
\begin{equation}
   \mathcal{I}(\omega) =  I_{-\frac{2}{3} i z_h \omega }\left(i\frac{\sqrt{z-z_h} \sqrt{8 \pi ^2 \omega ^2
   z_h^2+18 N^2 q^2 s \Gamma \left(\frac{2}{3}\right)^6 z_h^2+18 \pi ^2}}{3 \pi }\right)\,.
\end{equation}
Expanding \ref{eq:axprobenh} near the horizon, we find that the leading term of asymptotic expression $\alpha_h(z)$ takes
\begin{equation} \label{eq:alphanh}
\alpha_h(z) \sim A_h \left(12 \pi^2\right)^{\frac{i \omega z_h}{3}} \Bigg\lbrace\left(z_h -z\right) \left[9 N^2 q^2 s z_h^2 \Gamma
   \left(\frac{2}{3}\right)^6+\pi ^2 \left(4 \omega^2 z_h^2+9\right)\right]\Bigg\rbrace^{1/2 -i \omega z_h/3}
\end{equation} 
where $A_h$ is some normalization constant. Using the relation of the conservative current \ref{eq:jcons}, we obtain
\begin{equation}\label{eq:g}
{\rm Im}G_R(\omega)=\frac{|A_h|^2}{|\alpha_0|^2}\frac{z_h\omega}{3\pi^2}\left[9N^2q^2sz_h^2\Gamma\left(\frac23\right)^6+\pi^2(4z_h^2\omega^2+9)\right]\,,  
\end{equation}
In order to acquire the exact expression of the retarded Green function, we need to fix the ratio $|A_h|^2/|\alpha_0|^2$, and further apply the Kramers-Kronig relation. We tried to solve the equation of $a(z)$ in the $N\to 0$ limit, namely the pure AdS solution, which can be derived analytically throughout the whole radial coordinate 
\begin{equation}\label{eq:a1ads}
a(z)=C\,e^{i\frac{\sqrt{3}}{3}z_h\omega\arctan(\frac{2z+z_h}{\sqrt{3}z_h})}(z^2+z_hz+z_h^2)^{\frac{i}{6}z_h\omega}(z_h-z)^{-\frac{i z_h\omega}{3}} \,. 
\end{equation}
And then, we intended to match the ratio $|A_h|^2/|\alpha_0|^2$ for pure AdS case with the one in the presence of $N$. However, the issue is that this practice ignores the contribution of $N$ to the ratio and the freedom of the coefficient $A_h$ can not be fixed. 

%in such a way that \ref{eq:alphanh} smoothly connects to \ref{eq:a1ads} in absence of a scalar field. After this, we find
%\begin{equation}\label{eq:a1ads}
%{\rm Im}[g] =  w \left[1+\frac{9 N^2 q^2 s z_h^2 \Gamma\left(\frac{2}{3}\right)^6}{\pi^2 \left(4 \omega^2 z_h^2 +9\right)}\right]\,.
%\end{equation}
%The full retarded Green function $G_R$ can be obtained by following \ref{eq:Gr}, which reads
%\begin{equation} \label{eq:GRprobe}
%    G_R(\omega) = i \omega + \frac{9 N^2 q^2 s \Gamma \left(\frac{2}{3}\right)^6}{4 \pi ^2 (2 \pi  T- i \omega )}\,.
%\end{equation}

%To compute the conductivity, we need to evaluate the formula \ref{eq:sigma}. This can be done by applying the Sokhotski–Plemelj theorem, 
%\begin{equation} 
%\lim_{\delta\to 0} \frac{1}{x+\delta i} = \mathcal{P}\left[\frac{1}{x}\right] -i \pi \delta(x)\,,
%\end{equation} 
%where $\mathcal{P}$ stands for the principal value. After this, we find
%\begin{equation}\label{eq:sigmaprobe}
%\sigma = \left[1 +\frac{9 N^2 q^2 s \Gamma
%   \left(\frac{2}{3}\right)^6}{4 \pi^2 \left(4 \pi ^2 T^2+\omega
%   ^2\right)} - \frac{9 N^2 q^2 s \Gamma
%   \left(\frac{2}{3}\right)^6}{8 \pi^2 T}\delta\left(\omega\right) \right] - i  \frac{9 N^2 q^2 s T \Gamma\left(\frac{2}{3}\right)^6}{2\pi\omega\left(4\pi^2 %T^2+\omega^2\right)}  \,.
%\end{equation} 
%From \ref{eq:sigmaprobe}, it is straightforward to compute the weight spectral distribution, which reads
%\begin{equation} 
%W(\omega) = \frac{9 N^2 q^2 s \Gamma \left(\frac{2}{3}\right)^6}{8 \pi ^2 T} F(\omega) \,, \quad F(\omega) = 1+ \frac{1}{\pi}\cot ^{-1}\left(\frac{2 \pi  %T}{\omega }\right) -2\theta(\omega)
%\end{equation} 
%where $\theta(\omega)$ stands for the Heavyside function. In particular, $F<0 \,\forall \,\omega>0$, so the overall sign of $W$ is determined by $s$ alone. %In particular, when $x>1$, $W<0$ and $>0$ if otherwise. Furthermore, the sum rule, 
%\begin{equation} \label{eq:intresigma}
%    \int^\infty_{-\infty} \big\lbrace {\rm Re}[\sigma] - 1 \big\rbrace \, d\omega = 0\,,
%\end{equation}
%is always satisfied. Moreover, notice that it requires a finite coupling strength between the gauge field and the scalar field, i.e. $q\neq 0$ in order to %see any scalar field contribution to the longitudinal conductivity \ref{eq:sigmaprobe}, as expected.

==> backup/questions.tex <==
\documentc'lass[12pt]{letter}
\usepackage{graphicx}
\usepackage{geometry}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{color}
\usepackage{dcolumn}
\usepackage{slashed}
\usepackage{ulem}
\newcommand{\red}[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\newcommand{\blue}[1]{{\leavevmode\color[rgb]{0.33,0.33,1.00}{#1}}}
\newcommand{\green}{\textcolor[rgb]{0.13,0.62,0.16}}
\newcommand{\purple}{\textcolor[rgb]{0.44,0.00,0.94}}
\usepackage{comment}
\usepackage{xcolor}

\geometry{left=3.0cm,right=3.0cm,top=2.8cm,bottom=2.8cm}

\newcommand{\StyleReferee}{\it}
\newcommand{\StyleAuthor}{}


\def\P{\mathcal{P}}
\def\T{\mathcal{T}}
\def\PT{\mathcal{PT}}
\def\TP{\mathcal{TP}}

\newcounter{mycounter}
% \setcounter{mycounter}{1}

\begin{document}

\begin{flushleft}
Dear Daniel and Karl,
\end{flushleft}

We had the follwoing questions on your interesting paper [1]:
\begin{itemize}
    \item Why do you consider the initial gauge $\phi=e^{i\alpha}\tilde M, \bar\phi=e^{-i\alpha}\tilde M$ instead of  $\phi=e^{i\alpha}\tilde M, \bar\phi=e^{-i\alpha}\tilde M^*$ ? Similarly, why do you consider the ansatz
   $
        \phi=(1-x)\psi,\, \bar\phi=(1+x)\psi
    $
    in Eq.~(13) of [1], instead of 
    $
        \phi=(1-x)\psi,\, \bar\phi=(1+x)\psi^*
    $? Our concern is: If your solutions become complex for $x>1$, you may not be able to sustain this gauge any longer. Do you know what happens then?
    \item On the complex solutions in the $\PT$-broken phase with $x>x_c>1$ in either $T=0$ case or $T>0$ case, we have several questions: Why is the geometry complex? The energy-momentum tensor in the bulk depends on the absolute value of the scalar, so shouldn't the geometry be real? How does one define the temperature when the metric is complex, and why do you  get a real $M/T$? Are the complex solutions stable or not?
    \item How do $\P,\, \T$ and $\PT$ transform the fields? The transformations in [1] look slightly different from the transformations in appendix A of [2]. Is the transformation $x_1\to-x_1$ in $\P$ always necessary to define the $\PT$ transformation?
\end{itemize}

With Best Regards,

Daniel, Ren\'e, Yang, Zhaohui and Zhuo-Yu.

[1]
%\cite{Arean:2019pom}
% \bibitem{Arean:2019pom}
D.~Are\'an, K.~Landsteiner and I.~Salazar Landea,
``Non-hermitian holography,''
SciPost Phys. \textbf{9}, no.3, 032 (2020)
% doi:10.21468/SciPostPhys.9.3.032
[arXiv:1912.06647 [hep-th]].
%11 citations counted in INSPIRE as of 19 Nov 2022

[2]
%\cite{Morales-Tejera:2022hyq}
% \bibitem{Morales-Tejera:2022hyq}
S.~Morales-Tejera and K.~Landsteiner,
``Non-Hermitian Quantum Quenches in Holography,''
[arXiv:2203.02524 [hep-th]].
%1 citations counted in INSPIRE as of 19 Nov 2022

\end{document}

